EntroGD: Scalable Generalized Deduplication for Efficient Direct Analytics on Compressed IoT Data

Massive data streams from IoT and cyber-physical systems must be processed under strict bandwidth, latency, and resource constraints. Generalized Deduplication (GD) is a promising lossless compression framework, as it supports random access and direct analytics on compressed data. However, existing GD algorithms exhibit quadratic complexity $\mathcal{O}(nd^{2})$, which limits their scalability for high-dimensional datasets. This paper proposes \textbf{EntroGD}, an entropy-guided GD framework that decouples analytical fidelity from compression efficiency to achieve linear complexity $\mathcal{O}(nd)$. EntroGD adopts a two-stage design, first constructing compact condensed samples to preserve information critical for analytics, and then applying entropy-based bit selection to maximize compression. Experiments on 18 IoT datasets show that EntroGD reduces configuration time by up to $53.5\times$ compared to state-of-the-art GD compressors. Moreover, by enabling analytics with access to only $2.6\%$ of the original data volume, EntroGD accelerates clustering by up to $31.6\times$ with negligible loss in accuracy. Overall, EntroGD provides a scalable and system-efficient solution for direct analytics on compressed IoT data.

==> algorithm_customisations.tex <==
% Code to make vertical lines in algorithmic
% source: https://tex.stackexchange.com/a/524700
\makeatletter
% This is the vertical rule that is inserted
\newcommand*{\algrule}[1][\algorithmicindent]{%
    \hspace*{.5em}% <------------- This is where the rule starts from
    \vrule %height .75\baselineskip depth .25\baselineskip
    \hspace*{\dimexpr#1-.2em-.4pt}%
}

\newcommand{\StatePar}[1]{%
    \State\parbox[t]{\dimexpr\linewidth-\ALG@thistlm}{\strut #1\strut}%
}
\renewcommand{\ALG@beginalgorithmic}{\offinterlineskip}% Remove all interline skips

\newcount\ALG@printindent@tempcnta
\def\ALG@printindent{%
    \ifnum \theALG@nested > 0% is there anything to print
    \ifx\ALG@text\ALG@x@notext% is this an end group without any text?
    % do nothing
    \else
    \unskip
    % draw a rule for each indent level
    \ALG@printindent@tempcnta=1
    \loop
    \algrule[\csname ALG@ind@\the\ALG@printindent@tempcnta\endcsname]%
    \advance \ALG@printindent@tempcnta 1
    \ifnum \ALG@printindent@tempcnta<\numexpr\theALG@nested+1\relax
    \repeat
    \fi
    \fi
}
% the following line injects our new indent handling code in place of the default spacing
\patchcmd{\ALG@doentity}{\noindent\hskip\ALG@tlm}{\ALG@printindent}{}{\errmessage{failed to patch}}
% end vertical rule patch for algorithmicx
\makeatother

% Add \struts to keywords
\algrenewcommand\algorithmicend{\strut\textbf{end}}
\algrenewcommand\algorithmicdo{\strut\textbf{do}}
\algrenewcommand\algorithmicwhile{\strut\textbf{while}}
\algrenewcommand\algorithmicfor{\strut\textbf{for}}
\algrenewcommand\algorithmicforall{\strut\textbf{for all}}
\algrenewcommand\algorithmicloop{\strut\textbf{loop}}
\algrenewcommand\algorithmicrepeat{\strut\textbf{repeat}}
\algrenewcommand\algorithmicuntil{\strut\textbf{until}}
\algrenewcommand\algorithmicprocedure{\strut\textbf{procedure}}
\algrenewcommand\algorithmicfunction{\strut\textbf{function}}
\algrenewcommand\algorithmicif{\strut\textbf{if}}
\algrenewcommand\algorithmicthen{\strut\textbf{then}}
\algrenewcommand\algorithmicelse{\strut\textbf{else}}

\algrenewcommand\algorithmicrequire{\strut\textbf{Input:}}
\algrenewcommand\algorithmicensure{\strut\textbf{Output:}}

\let\oldState\State
\renewcommand{\State}{\oldState\strut}

